TD Convergence: An Optimization Perspective

We study the convergence behavior of the celebrated temporal-difference (TD) learning algorithm. By looking at the algorithm through the lens of optimization, we first argue that TD can be viewed as an iterative optimization algorithm where the function to be minimized changes per iteration. By carefully investigating the divergence displayed by TD on a classical counter example, we identify two forces that determine the convergent or divergent behavior of the algorithm. We next formalize our discovery in the linear TD setting with quadratic loss and prove that convergence of TD hinges on the interplay between these two forces. We extend this optimization perspective to prove convergence of TD in a much broader setting than just linear approximation and squared loss. Our results provide a theoretical explanation for the successful application of TD in reinforcement learning.

==> future_directions.tex <==
\section{Future Directions}

==> outline.tex <==
\section{Outline}
\begin{enumerate}
    \item related work distill known TD issues/convergence guarantees
    \item intro (a few words about TD, deadly triad, bootstrapping), talk about the offline setting. what is our contribution.
    \item background
    \item start with the TD update, and then connect it to the particular H
    \item counter example? the factor lipschitzness of objective (intuitive level)
    \item linear case (start with van roy tsiklis) and then we prove our result about spectral radius
    \item generalized H (Huber loss, logistic regression, ... , different function approximator, such as decision trees) fitted value iteration
    \item prove for generalized H exact case
    \item nested case for generalized H
    
\end{enumerate}

==> rebuttal/RevisedRelatedWork.tex <==
\section{Revised Related Work}


%In this paper, we studied convergence of TD through the lens of optimization. The underlying principles of TD are so central to RL that a large number of RL algorithms can be thought of as versions of TD, and the availability of convergence results varies between different types of algorithms. We chose a setting we believe is as elementary as possible to highlight key principles of TD convergence. Closest to our work is the work of Tsitsiklis and Van Roy \cite{tsitsiklis1996analysis} who proved convergence of TD with linear function approximation, squared loss, and the stationary-state distribution of the Markov chain. Later work further analyzed the finite-time convergence of TD with linear function approximation and squared loss~\cite{bhandari2018finite}, and also generalized it to the control setting~\cite{melo2008analysis, zou2019finite}.



% This paper deals with the convergence properties of pure TD for evaluation.  Despite the wide-spread use of TD methods in RL, convergence results are known mostly in special cases.  analyze the case for linear function approximation. \cite{bhandari2018finite} further study the finite-sample results of TD with on-policy samples and updating the target parameter at every step ($K=1$ for the inner optimization problem). In the non-linear case \citet{ollivier2018approximate} have proved convergence results for reversible policies with non-linear function approximation.
%Modifications of TD are presented in prior work that are more conducive to convergence analysis~\cite{sutton2016emphatic,zhang2021breaking, diddigi2019convergent,lim2022regularized, ghiassian2020gradient}. They have had varying degrees of success both in terms of empirical performance~\cite{ghiassian2017first}, and in terms of producing convergent algorithms~\cite{manek2022pitfalls}. TD is also studied under over-parameterization~\cite{cai2019neural, xiao2021understanding}, with learned representations~\cite{ghosh2020representations}, proximal updates~\cite{asadi2022faster}, and auxiliary tasks~\cite{lyle2021effect}. Also, the quality of TD fixed-point has been studied in previous work~\cite{kolter2011fixed}.

%A large body of literature focuses on finding TD-like approaches that are in fact true gradient-descent approaches in that they follow the gradient of a stationary objective function~\cite{sutton2009fast, maei2010toward,liu2012regularized, liu2016proximal,liu2020finite,feng2019kernel}. In these works, the optimization problem is formulated in such a way that the minimizer of the loss will be the fixed-point of the standard TD. Whereas TD has been extended to large-scale settings, these algorithms have not been as successful as TD in terms of applications.

%A closely related algorithm to TD is that of Baird, namely the residual gradient algorithm~\cite{baird1995residual, antos2008learning}. This algorithm has a double-sampling issue that needs to be addressed either by assuming a model of the environment or by learning the variance of the value function~\cite{antos2008learning, dai2018sbeed}. However, even with deterministic MDPs, in which the double sampling issue is not present~\cite{saleh2019deterministic}, the algorithm often finds a fixed-point that has a lower quality than that of the TD algorithm~\cite{lagoudakis2003least}. This is attributed to the fact that the MDP might still look stochastic in light of the use of function approximation~\cite{sutton2009fast}.

%TD could be thought of as an incremental approach to approximate dynamic programming and Fitted Value Iteration~\cite{gordon1995stable} for which various convergence results based on the operator view exits~\cite{ernst2005tree,lizotte2011convergent,fan2020theoretical}. Also, these algorithm are well-studied in terms of their error-propagation behavior~\cite{munos2007performance, munos2008finite, farahmand2010error}.

%Many asymptotic or finite-sample results on Q-learning (the control version of TD) with function approximation make additional assumptions on the problem structure, with a focus on the exploration problems in MDP \cite{jin2020provably, du2019provably, du2020agnostic, agarwal2020flambe, chen2020zap}. Like mentioned before, our focus was on the prediction setting where exploration is not relevant. 

We believe to be the first paper to show a exact contraction for TD with frozen target network and general $K$. To elaborate further, to the best of our knowledge, existing results prior to \cite{lee2019target} mainly considered the case where we either never freeze the target network (corresponding to the value of $K=1$), or the somewhat unrealistic case where we can exactly solve each iteration. Lee and He (2019) showed guarantees pertaining to the more general case of finite $K>1$, but notice that, while their result is quite innovative, they leaned on the more standard optimization tools for ensuring that gradient descent with a fixed $K$ can only solve each iteration approximately. Therefore, each iteration results in some error. In their theory, this error is accumulated per iteration and needs to be accounted for in the final result. Therefore, they fell short of showing 1) contraction and 2) exact convergence to the TD fixed-point, and only show that the final iterate is in the vicinity of the fixed-point defined by the amount of error accumulated over the trajectory. Another way to think about their result is that they can only show contraction if one uses gradient descent with infinite $K$ (which corresponds to exactly solving each iteration). With finite $K$, they need to account for errors in solving each iteration (denoted by $\epsilon_{k}$ in their proofs such as in Theorem 3), which prevent them from obtaining a clean convergence result. To better make the point, suppose that we solve the first iteration with some error, meaning that we approximately solve:
$$\theta^{1} \approx \arg\min_{w} H(\theta^0,w),$$
but then after we solve each iteration perfectly, meaning for $i\geq 1$:
$$\theta^{i+1} =  \arg\min_{w} H(\theta^i,w).$$
Clearly, one can think of approximately solving the first iteration as initializing TD to a point different than $\theta_0$ and then doing perfect optimization in all iterations. The fact that we then can solve each subsequent iteration perfectly should give us exactly a contraction to the TD fixed-point based on our analysis. However, in this case the result of Lee and He (2019) can still only support convergence to a neighborhood characterized by the approximation error $\varepsilon$. In contrast, in this case we can guarantee convergence exactly to the TD fixed-point. The part where they got stuck is where they use the more classical analysis that gradient descent only approximately solves each iteration, and so they need to accumulate some error along the way. In contrast, we can show that even approximately solving each iteration (corresponding to finite $K$) is enough to obtain contraction (without any error term), because we account for the progress of each gradient step towards the TD fixed-point.


%In terms of comparison with Zhang et al. (2021) and Chen et al. (2022), notice that due to the difficulties pertaining to proving convergence for vanilla TD, a line of existing research was to equip TD with modifications to make it more conducive to convergence. In this case, Zhang et al. (2021) introduced two projection steps that are crucial for obtaining convergence, and similarly Chen et al. (2022) studies the case where a truncation step is added. These are very important techniques, and they indeed can make TD more convergent. However, we were able to obtain a general result shows that vanilla TD converges with any value of $K$, and it also supports TD convergence in a broader setting. More precisely, our convergence result does not lean on these projection and truncation steps and is applicable to vanilla TD as well as TD with alternative loss functions and function approximators.

%Thanks for bringing the work of Melo et al (2008) into our attention. While we did cite this paper in our original submission (reference [22]), we agree that a more nuanced discussion about this important paper is warranted. We distill the key differences here, and in particular we discuss the similarity between their condition (7) and our condition. This discussion will be added to the paper.

%First, we understand the key contribution of \cite{melo2008analysis} to be the extension of the ODE proof of Tsitsiklis and Van Roy \cite{tsitsiklis1996analysis} from TD prediction to the more general control setting with Q-learning. Melo et al. show that asymptotically and under mild assumptions, the Q-learning algorithm with linear function approximation, quadratic loss, and $K = 1$ converges to a fixed-point.

%In this context, the condition in their equation (7) is in fact quite different than the condition identified in our paper. In their equation (7), they require that the eigenvalues of $\Sigma_{\pi}$, the policy-conditioned covariance matrix $\Phi^{\top}D\Phi$, dominate the eigenvalues of a second matrix $\gamma^{2}\Sigma_{\pi}^{\star}(\theta)$. Here $\Sigma_{\pi}^{\star}(\theta)$ is a similar covariance matrix for features, but one that is computed based on the action-greedification step.

%While this condition may look similar, a deeper investigation reveals that it is completely different from our condition. To recap, our condition requires that the optimization force (namely the same covariance matrix of the features) dominate the target force. In this case, the target force is defined as the degree to which the objective function $H$ can be affected by the target network variable. In the linear case, it depends on the eigenvalues of the matrix $\gamma\Phi^{\top}D\Phi$. Notice that this target force is governed, in part, by the transition matrix $P$. This is a major distinction between our condition and that of Melo et al. whose condition does not depend on $P$, and intuitively, their condition is more related to choosing the feature matrix $\Phi$ in such a way as to contain the negative effects due to maximization. To conclude, because the conditions are inherently different, the $\gamma^{2}$ factor in their result cannot be thought of as offering any particular advantage relative to our result.

%Moving from the condition itself, a major difference is present in the final guarantees obtained by us relative to Melo et al. In our case, we are interested in finding a finite-time contraction result, meaning that after each outer iteration $t$, we would like to provide a guarantee on the quality of the iterate we find relative to the TD fixed-point, whereas Melo et al. showed the somewhat weaker asymptotic convergence.

%Moreover, our results are better grounded in the empirical side of the RL literature in two important ways, namely 1) our results support the now ubiquitous deep RL practice of freezing the target network (which corresponds to the case of $K > 1$) whereas Melo et al. study the case of $K = 1$, and 2) we generalized the function class beyond the case of just linear functions and quadratic loss, and support a more abstract function class $H(\theta , w)$. This abstract class includes the setting studied by the important work of Melo et al. as a special case, but our setting also includes other interesting examples as explained in our general rebuttal.


%Moreover, in light of the more practical literature on TD where a finite $K$ is used, we were interested to show that 1) we converge to the TD fixed-point exactly and 2) with any value of $K$ the TD algorithm would give us a contraction. We indeed show in our main result that TD is a contraction with any value of $K$ (which we believe we are the first paper to show). More concretely, we show that smaller values of $K$ can damage the contraction factor, but each iteration will nevertheless remain contractive irregardless of $K$.

==> rest.tex <==
\section{Convergence of Linear TD in the On-policy case}
We first define the projection operator onto a plane as follows:
$$\Pi(v) = \arg\min_{v'=\Phi w}||v - v'||_{D}$$
Note that $\Pi(v)$ is a non-expansion:
$$\forall v,v'\quad ||\Pi(v)-\Pi(v')||_{D}\leq ||v - v'||_{D}$$
Proof of this can be found in standard textbooks, which relies on the variational characterization of projection. We then define the Bellman Operator:

$$T(v) = R + \gamma P v$$
Bellman operator is a $\gamma$ contraction under the $||\cdot||_{D}$ norm. To show this, we need the following lemma:
\begin{lemma}[Jensen's Inequality with Transition Matrices] For any vector $v$ and transition matrix $P$, we have
    $$||P v||_{D}\leq ||v||_{D}$$
\end{lemma}
\begin{proof}
    \begin{eqnarray*}
    ||P v||^2_{D} &=& (Pv)^{\top}D Pv\\
    &=&\sum_{i} D(i) (\sum_{j} P_{ij}v_j)^2\\
    &\leq &\sum_{i} D(i) \sum_{j} P_{ij}(v_j)^2\\
    &=&\sum_{j}(v_j)^2\sum_{i} D(i)P_{ij}\\
    &=&\sum_{j}D(j)(v_j)^2=||v||^2_D\\
    \end{eqnarray*}
where we used the Jensen's inequality. Also, the one before last equality is because of a property of the stationary-state distribution, namely that for any $j$ we have:
$\sum_{i} D(i) P_{ij}= D(j) $.
\end{proof}
\begin{lemma}[Bellman Contraction]
    $$||T v - T v'||_{D}\leq \gamma||v-v'||_{D}$$
\end{lemma}
\begin{proof}
   $$||T v - T v'||_{D} = ||R+\gamma P v - R + \gamma P v'||_{D} = ||\gamma P v - \gamma P v'||_{D}=\gamma  ||P(v- v')||_{D} \leq \gamma ||v- v'||_{D}$$
   where the inequality is due to the previous lemma.
\end{proof}
Now suppose we have:
$$w_{t+1} \leftarrow \arg\min_{w} h(w^{t},w)$$
which could be written as: 
\begin{eqnarray*}
w^{t+1}&=&\arg\min_{w} h(w^{t},w)\\
&=& \arg\min_{w}||R+\gamma P \Phi w^{t} - \Phi w||_{D} \\
&=& \arg\min_{w} ||T(\Phi w^{t}) -\Phi w||_{D}
\end{eqnarray*}
Because $\Phi$ has linearly independent columns, we can write the iterations above as:
\begin{eqnarray*}
\Phi w^{t+1}&=& \arg\min_{v: v = \Phi w} ||T(\Phi w^{t}) -v||_{D}\\
&=&\Pi_{D}\big(T(\Phi w^{t})\big)
\end{eqnarray*}
Recall that $\Pi_{D}$ is a non-expansion in $||\cdot||_{D}$ and that $T$ is a $\gamma$-contraction in $||\cdot||_{D}$, therefore $\Pi_{D}\big(T(\cdot))$ is a $\gamma$-contraction in  $||\cdot||_{D}$. This point could be characterized by:
$$\Phi w^{\star} = \Pi_{D}\big(T(\Phi w^{\star})\big)$$

\section{Non-Prox Convergence Rate Results}
Given an RL loss function $h : \mathbb{R}^{n} \times \mathbb{R}^{n} \rightarrow \mathbb{R}$, we are interested in finding $w^{\star}$, which satisfy the following optimality condition
\begin{equation} \label{Optimality}
    \nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}.
\end{equation}
Here, we will focus on the following class of algorithms:
\begin{equation} \label{Algo:Exact}
    w^{t + 1} \leftarrow \arg\min_{w} h(w^{t} , w).
\end{equation}
We begin with the proof of the exact approach, which is stated next.
\begin{theorem}[Contraction - Exact approach]
    Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by Algorithm \eqref{Algo:Exact}. Suppose that $w^{\star}$ is any point satisfying the condition $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$, then for any $t \in \mathbb{N}$, we have the following contraction property
    \begin{equation*}
        \|w^{t + 1} - w^{\star}\| \leq \underbrace{\frac{L_{1}}{\mu_2}}_{:=\eta}\|w^{t} - w^{\star}\|.
    \end{equation*}
\end{theorem}
\begin{proof}
From \eqref{Algo:Exact}, it immediately follows that $\nabla_{2} h(w^{t} , w^{t + 1}) = {\bf 0}$. Now, using the $\mu_{2}$-strong convexity of $w \rightarrow h(w^{t} , w)$, we get that
\begin{equation*}
    \mu_{2}\|w^{t + 1} - w^{\star}\|^{2} \leq \langle w^{\star} - w^{t + 1} , \nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{t} , w^{t + 1}) \rangle = \langle w^{\star} - w^{t + 1} , \nabla_{2} h(w^{t} , w^{\star}) \rangle.
\end{equation*}
Now, since $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$, we obtain from the Cauchy-Schwartz inequality that
\begin{align*}
    \mu_{2}\|w^{t + 1} - w^{\star}\|^{2} & \leq \langle w^{\star} - w^{t + 1} , \nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star}) \rangle \\
    & \leq \|w^{t + 1} - w^{\star}\| \cdot \|\nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star})\| \\
    & \leq L_{1}\|w^{t + 1} - w^{\star}\| \cdot \|w^{t} - w^{\star}\|,    
\end{align*}
where the last inequality follows from the $L_{1}$-Lipschitz property of $\nabla_{2} h(\cdot,w^{\star})$. Since this inequality holds true for any $t \in \mathbb{N}$, we see that if $w^{t} = w^{\star}$, then also $w^{t + 1} = w^{\ast}$. Thus, if $w^{T} = w^{\star}$ for some $T \in \mathbb{N}$, then $w^{t} = w^{\ast}$ for any $t \geq T$. On the other hand, if $w^{t} \neq w^{\ast}$ for all $t \in \mathbb{N}$, the desired result follows after dividing both sides by $\|w^{t + 1} - w^{\ast}\|$.
\end{proof}
Now, we continue with the nested case. The inner iteration are given by
\begin{equation*}
    w^{t,k+1} \leftarrow w^{t,k} - \alpha\nabla_2 h(w^t,w^{t,k}).
\end{equation*}

In order to prove a contraction property in this case, we will need the following two technical results. 
\begin{proposition} \label{P:Tech1}
    Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by Nested TD. Then, for all $t \in \mathbb{N}$ and $0 \leq k \leq K - 1$, we have
\begin{equation*}
    h(w^{t} , w^{\star}) - h(w^{t} , w^{t,k}) \leq \frac{L_{1}^{2}}{2\mu_{2}}\|w^{t} - w^{\star}\|^{2} - \left(\frac{1}{\alpha} - \frac{L_{2}}{2}\right)\|w^{t,k + 1} - w^{t,k}\|^{2}.
\end{equation*}
\end{proposition}
\begin{proof}
Let $t \in \mathbb{N}$. From the $\mu_{2}$-strong convexity of $w \rightarrow h(w^{t} , w)$, we obtain that
\begin{equation*}
    h(w^{t} , w^{t,k + 1}) \geq h(w^{t} , w^{\star}) + \langle \nabla_{2} h(w^{t} , w^{\star}) , w^{t,k + 1} -  w^{\star}\rangle + \frac{\mu_{2}}{2}\|w^{t,k + 1} - w^{\star}\|^{2},
\end{equation*}
which means that
\begin{equation} \label{P:Tech1:1}
    h(w^{t} , w^{\star}) - h(w^{t} , w^{t,k + 1}) \leq \langle \nabla_{2} h(w^{t} , w^{\star}) , w^{\star} - w^{t,k + 1}\rangle - \frac{\mu_{2}}{2}\|w^{t,k + 1} - w^{\star}\|^{2}.
\end{equation}
Moreover, from the fact that $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$, we have
\begin{align}
    \langle \nabla_{2} h(w^{t} , w^{\star}) , w^{\star} - w^{t,k + 1}\rangle & = \langle \nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star}) , w^{\star} - w^{t,k + 1}\rangle \nonumber \\
    & \leq \frac{1}{2\mu_{2}}\|\nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star})\|^{2} + \frac{\mu_{2}}{2}\|w^{t,k + 1} - w^{\star}\|^{2} \nonumber \\
    & \leq \frac{L_{1}^{2}}{2\mu_{2}}\|w^{t} - w^{\star}\|^{2} + \frac{\mu_{2}}{2}\|w^{t,k + 1} - w^{\star}\|^{2},  \label{P:Tech1:2}
\end{align}
where the first inequality follows from the simple fact that $a^{T}b \leq (1/2d)\|a\|^{2} + (d/2)\||b\|^{2}$ for any $d > 0$ and in our case, we take $d = \mu_{2}$, while the last inequality follows from the Lipschitz property of the gradient. Hence, by combining  \eqref{P:Tech1:1} with \eqref{P:Tech1:2}
\begin{align*}
    h(w^{t} , w^{\star}) - h(w^{t} , w^{t,k + 1}) & \leq \frac{L_{1}^{2}}{2\mu_{2}}\|w^{t} - w^{\star}\|^{2} + \frac{\mu_{2}}{2}\|w^{t,k + 1} - w^{\star}\|^{2} - \frac{\mu_{2}}{2}\|w^{t,k + 1} - w^{\star}\|^{2} \\
    & = \frac{L_{1}^{2}}{2\mu_{2}}\|w^{t} - w^{\star}\|^{2}.
\end{align*}
From the Descent Lemma, we have
\begin{align*}
    h(w^{t} , w^{t,k + 1}) & \leq h(w^{t} , w^{t,k}) + \langle \nabla_{2} h(w^{t} , w^{t,k}) , w^{t,k + 1} -  w^{t,k}\rangle + \frac{L_{2}}{2}\|w^{t,k + 1} - w^{t,k}\|^{2} \\
    & = h(w^{t} , w^{t,k}) + \frac{1}{\alpha}\langle w^{t,k} - w^{t,k + 1} , w^{t,k + 1} -  w^{t,k}\rangle + \frac{L_{2}}{2}\|w^{t,k + 1} - w^{t,k}\|^{2} \\
    & = h(w^{t} , w^{t,k}) - \left(\frac{1}{\alpha} - \frac{L_{2}}{2}\right)\|w^{t,k + 1} - w^{t,k}\|^{2}.
\end{align*}
Combining both previous inequalities yields
\begin{equation*}
    h(w^{t} , w^{\star}) - h(w^{t} , w^{t,k}) \leq \frac{L_{1}^{2}}{2\mu_{2}}\|w^{t} - w^{\star}\|^{2} - \left(\frac{1}{\alpha} - \frac{L_{2}}{2}\right)\|w^{t,k + 1} - w^{t,k}\|^{2},
\end{equation*}
which proves the desired result.
\end{proof}
Now, we can prove the following result.
\begin{proposition} \label{P:Tech2}
    Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by Nested TD. Then, for all $t \in \mathbb{N}$ and $0 \leq k \leq K - 1$, we have
\begin{equation*}
    \|w^{t,k + 1} - w^{\star}\|^{2} \leq \left(1 - \alpha\mu_{2}\right)\|w^{t,k} - w^{\star}\|^{2} + \frac{\alpha L_{1}^{2}}{\mu_{2}}\|w^{t} - w^{\star}\|^{2} - \left(1 - \alpha L_{2}\right)\|w^{t,k + 1} - w^{t,k}\|^{2}.
\end{equation*}
In particular, when $\alpha = 1/L_{2}$, we have
\begin{equation*}
    \|w^{t,k + 1} - w^{\star}\|^{2} \leq \left(1 - \frac{\mu_{2}}{L_{2}}\right)\|w^{t,k} - w^{\star}\|^{2} + \frac{L_{1}^{2}}{L_{2}\mu_{2}}\|w^{t} - w^{\star}\|^{2}.
\end{equation*}
\end{proposition}          
\begin{proof}
Let $t \in \mathbb{N}$. From the definition of the inner iterations, for any $0 \leq k \leq K - 1$, we obtain that
\begin{equation*}
    \|w^{t,k + 1} - w^{\star}\|^{2} = \|w^{t,k} - w^{\star}\|^{2} + 2\alpha\langle \nabla_{2} h\left(w^{t} , w^{t,k}\right) , w^{\star} - w^{t,k}\rangle + \|w^{t,k + 1} - w^{t,k}\|^{2}.
\end{equation*}
Using the $\mu_{2}$-strong convexity of $w \rightarrow h(w^{t} , w)$, we have
\begin{equation*}
    h\left(w^{t} , w^{\star}\right) \geq h\left(w^{t} , w^{t,k}\right) + \langle \nabla_{2} h\left(w^{t} , w^{t,k}\right) , w^{\star} - w^{t,k}\rangle + \frac{\mu_{2}}{2}\|w^{t,k} - w^{\star}\|^{2},
\end{equation*}
which combined with the inequality above yields that
\begin{align*}
    \|w^{t,k + 1} - w^{\star}\|^{2} & \leq \|w^{t,k} - w^{\star}\|^{2} + 2\alpha\left(h\left(w^{t} , w^{\star}\right) - h\left(w^{t} , w^{t,k}\right) - \frac{\mu_{2}}{2}\|w^{t,k} - w^{\star}\|^{2}\right) + \|w^{t,k + 1} - w^{t,k}\|^{2} \\
    & = \left(1 - \alpha\mu_{2}\right)\|w^{t,k} - w^{\star}\|^{2} + 2\alpha\left(h\left(w^{t} , w^{\star}\right) - h\left(w^{t} , w^{t,k}\right)\right) + \|w^{t,k + 1} - w^{t,k}\|^{2}.
\end{align*}
Hence, from Proposition \ref{P:Tech1}, we obtain
\begin{align*}
    \|w^{t,k + 1} - w^{\star}\|^{2} & \leq \left(1 - \alpha\mu_{2}\right)\|w^{t,k} - w^{\star}\|^{2} + 2\alpha\left(\frac{L_{1}^{2}}{2\mu_{2}}\|w^{t} - w^{\star}\|^{2} - \left(\frac{1}{\alpha} - \frac{L_{2}}{2}\right)\|w^{t,k + 1} - w^{t,k}\|^{2}\right) \\
    & + \|w^{t,k + 1} - w^{t,k}\|^{2} \\
     & = \left(1 - \alpha\mu_{2}\right)\|w^{t,k} - w^{\star}\|^{2} + \frac{\alpha L_{1}^{2}}{\mu_{2}}\|w^{t} - w^{\star}\|^{2} - \left(1 - \alpha L_{2}\right)\|w^{t,k + 1} - w^{t,k}\|^{2},
\end{align*}
which completes the first desired result. By setting $\alpha = 1/L_{2}$, we obtain that 
\begin{equation*}
    \|w^{t,k + 1} - w^{\star}\|^{2} \leq \left(1 - \frac{\mu_{2}}{L_{2}}\right)\|w^{t,k} - w^{\star}\|^{2} + \frac{L_{1}^{2}}{L_{2}\mu_{2}}\|w^{t} - w^{\star}\|^{2},
\end{equation*}
which completes the proof.
\end{proof}

\section{Linear Approximation}
Here, we consider the following scenario 
\begin{equation*}
    h(\theta , w) = \frac{1}{2}\|R + \gamma P\Phi\theta - \Phi w\|^{2}_{D},
\end{equation*}
where $D \in \mathbb{R}^{n \times n}$ is a positive definite diagonal distribution matrix, $P \in \mathbb{R}^{n \times n}$ is a state transition matrix, and the feature matrix $\Phi \in \mathbb{R}^{n \times n}$ has linearly independent columns. In this case, we can prove the following result. Before, given a matrix $A \in \mathbb{R}^{n \times n}$, we just recall the notion of spectral radius of $A$, which is denoted by $\rho(A)$ and defined to largest eigenvalue in absolute value. 
\begin{proposition} \label{P:LinearTD}
    Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by TD. Then, for any vector $w^{\star} \in \mathbb{R}^{n}$ which satisfies $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$, we have 
    \begin{equation*}
        w^{t + 1} - w^{\star} = \gamma A\left(w^{t} - w^{\star}\right),
    \end{equation*}
    where $A := \left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi$. Moreover, $\{ w^{t} \}_{t \in \mathbb{N}}$ converges to $w^{\star}$ if and only if $\rho(A) < \gamma^{-1}$.
\end{proposition}
\begin{proof}
    From the definition of $h$, we obtain that
\begin{equation*}
    \nabla_{2} h(\theta , w) = -\Phi^{T}D\left(R + \gamma P\Phi\theta - \Phi w\right).
\end{equation*}    
Therefore, $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$ simply translates to $\Phi^{T}D\left(R + \gamma P\Phi w^{\star}\right) = \Phi^{T}D\Phi w^{\star}$, which can be equivalently written as follows 
\begin{equation} \label{P:LinearTD:1}
    \Phi^{T}D\left(I - \gamma P\right)\Phi w^{\star} = \Phi^{T}DR.
\end{equation}
Moreover, from the optimality of TD, we have 
\begin{equation*}
    \nabla_{2} h(w^{t} , w^{t + 1}) = {\bf 0},
\end{equation*}
which means that 
\begin{equation*}
    \Phi^{T}D\Phi w^{t + 1} = \Phi^{T}D\left(R + \gamma P\Phi w^{t}\right) = \Phi^{T}D\left(I - \gamma P\right)\Phi w^{\star} + \gamma \Phi^{T}DP\Phi w^{t},
\end{equation*}
where the last equality follows from \eqref{P:LinearTD:1}. Therefore, by rearranging this equality, we get that
\begin{equation*}
    \Phi^{T}D\Phi\left(w^{t + 1} - w^{\star}\right) = \gamma\Phi^{T}DP\Phi\left(w^{t} - w^{\star}\right),
\end{equation*}
which proves the desired result by inverting the positive definite matrix $\Phi^{T}D\Phi$. The second assertion follows from classical results \cite{}.
\end{proof}
From Proposition \ref{P:LinearTD} it follows that the convergence of TD in the setting of linear approximation is fully characterized by the spectral radius of the matrix $A$. Therefore, an immediate consequence of this result is the convergence of TD for the setting of no function approximation. 
\begin{corollary}[TD with no function approximation]
Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by TD with $\Phi = I$. Then, for any distribution matrix $D \in \mathbb{R}^{n \times n}$, the sequence $\{ w^{t} \}_{t \in \mathbb{N}}$ converges to a solution $w^{\star}$ satisfying $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$.
\end{corollary}
\begin{proof}
    From Proposition \ref{P:LinearTD}, it follows that in this case (recall that $\Phi = I$), then $A \equiv P$ and from classical results on stochastic matrices we know that $\rho(P) = 1$. Therefore, in this case, we have that $\rho(A) < \gamma^{-1}$ and TD always converges (for any matrix $D$) directly from Proposition \ref{P:LinearTD}.
\end{proof}
Recalling again the function $h$
\begin{equation*}
    h(\theta , w) = \frac{1}{2}\|R + \gamma P\Phi\theta - \Phi w\|^{2}_{D},
\end{equation*}
we obtain that 
\begin{equation*}
    \nabla_{2} h(\theta , w) = -\Phi^{T}D\left(R + \gamma P\Phi\theta - \Phi w\right).
\end{equation*}   
Therefore, as we obtained in the proof of Proposition \ref{P:LinearTD}, there are two matrices that play a central role in the convergence of TD, which are
\begin{equation*}
    B = \Phi^{T}DP\Phi \qquad \text{and} \qquad C = \Phi^{T}D\Phi.
\end{equation*}  
We obviously have that $A \equiv C^{-1}B$. Our goal is to show a few conditions on the individual matrices $B$ and $C$, which guarantee that $\rho(A) < \gamma^{-1}$, and therefore guarantee the convergence of TD. 
\begin{corollary}
Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by TD and assume that $\gamma\|B\|_{2} < \lambda_{min}(C)$. Then, the sequence $\{ w^{t} \}_{t \in \mathbb{N}}$ converges to a solution $w^{\star}$ satisfying $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$.
\end{corollary}
\begin{proof}
    From Proposition \ref{P:LinearTD} it is enough to show that in this case (recall that $\gamma \|B\|_{2} < \lambda_{min}(C)$), $\rho(A) < \gamma^{-1}$. For any matrix $X$ we have that $\rho(X) \leq \|X\|_{2}$, and therefore (recall that $A \equiv C^{-1}B$)
    \begin{equation*}
        \rho(A) \leq \|A\|_{2} = \|C^{-1}B\| \leq \|C^{-1}\| \cdot \|B\| <  \|C^{-1}\| \cdot \gamma^{-1}\lambda_{min}(C) = \gamma^{-1},
    \end{equation*}
    where the last equality follows from the fact that $\|C^{-1}\| = \lambda_{min}(C)^{-1}$ since $C \succ 0$ and symmetric.
\end{proof}



and we are interested in finding a vector $w^{\star}$ which satisfies $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$. In this case, it simply translates to $\Phi^{T}D\left(R + \gamma P\Phi w^{\star}\right) = \Phi^{T}D\Phi w^{\star}$. Equivalently, we can write $\Phi^{T}D\left(I - \gamma P\right)\Phi w^{\star} = \Phi^{T}DR$. From the optimality we have 
\begin{equation*}
    \nabla_{2} h(w^{t} , w^{t + 1}) = {\bf 0},
\end{equation*}
which means 
\begin{equation*}
    \Phi^{T}D\Phi w^{t + 1} = \Phi^{T}D\left(R + \gamma P\Phi w^{t}\right) = \Phi^{T}D\left(I - \gamma P\right)\Phi w^{\star} + \gamma \Phi^{T}DP\Phi w^{t},
\end{equation*}
that is
\begin{equation*}
    \Phi^{T}D\Phi\left(w^{t + 1} - w^{\star}\right) = \gamma\Phi^{T}DP\Phi\left(w^{t} - w^{\star}\right).
\end{equation*}
Therefore
\begin{equation*}
    w^{t + 1} - w^{\star} = \gamma\left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi\left(w^{t} - w^{\star}\right).
\end{equation*}
From the proofs in Section 2 above it follows that
\begin{equation*}
    I \succeq \left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi,
\end{equation*}
and now we need to prove that $L_{1} < \mu_{2}$. To this end, as long as $\Phi^{T}D\Phi \succ 0$, we can equivalently write it as follows
\begin{equation*}
    \Phi^{T}D\Phi \succeq \Phi^{T}DP\Phi,
\end{equation*}
\textbf{counter example}
We show that the condition $\forall i\ \lambda_{i}(C)>\lambda_{i}(B)$ does not guarantee $\lambda_{\max}(C^{-1}B)\leq 1$.\\
suppose $C= \left[ {\begin{array}{c c }
   \frac{3}{2} & 0  \\
   0 & \frac{5}{2}  \\
  \end{array} } \right]$ and $B= \left[ {\begin{array}{c c }
   2 & 0  \\
   0 & 1  \\
  \end{array} } \right]$ Notice that $\forall i\ \lambda_{i}(B)>\lambda_{i}(C)$. However, $C^{-1}B = \left[ {\begin{array}{c c }
   \frac{4}{3} & 0  \\
   0 & \frac{2}{5} \\
  \end{array} } \right]$ and so it is not true that $\lambda_{\max}(C^{-1}B)\leq 1$.


\begin{lemma}
Show that $-\lambda_{i}(\Phi^{T}D\Phi) < \lambda_{i}(\gamma\Phi^{T}DP\Phi)< \lambda_{i}(\Phi^{T}D\Phi) .$
\end{lemma}
\begin{proof}
Because $\gamma \left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi$ is a $\gamma$-contraction [citation], its eigenvalues must be between $-\gamma$ and $\gamma$, therefore we have that $I - \gamma\left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi$ is a positive-definite matrix:
\begin{equation*}
    I - \gamma\left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi> 0
\end{equation*}
The multiplication of two positive definite matrices is itself positive definite, which means that we can multiply both sides by another positive definite matrix $\Phi^{T}D\Phi$ and get the following:
\begin{equation*}
    \Phi^{T}D\Phi - \gamma\Phi^{T}DP\Phi> 0
\end{equation*}
Because this matrix is positive definite, it must be that:
$$\lambda_{i}(\Phi^{T}D\Phi) > \lambda_{i}(\gamma\Phi^{T}DP\Phi)\ ,$$
which is the desired result. Similarly, because $\gamma \left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi$ is a $\gamma$-contraction, we have that $-I - \gamma\left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi$ is a negative-definite matrix:
$$-I - \gamma\left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi<0 , $$
which means that:
\begin{equation*}
    \Phi^{T}D\Phi + \gamma\Phi^{T}DP\Phi = \Phi^{T}D\Phi - (-\gamma\Phi^{T}DP\Phi)>0
\end{equation*}
so it must be that
$$-\lambda_{i}(\Phi^{T}D\Phi) < \lambda_{i}(\gamma\Phi^{T}DP\Phi)\ ,$$
which combined with the first result completes the proof.
\end{proof}



We now the following about $D$:
$$\forall j\quad \sum_{i} D_{ii} P_{ij} = D_{jj}$$

$$ w^{t+1}\leftarrow\arg\min_{w} \sum_{s} D(s) h(w^{t}, w , s)$$
when solving this at each iteration, we will get:
$$\sum_{s} D(s)\nabla_{2} h(w^{t}, w^{t+1} , s) = {\bf 0}$$
and so the fixed point is:
$$\sum_{s} D(s)\nabla_{2} h(w^{\star}, w^{\star} , s) = {\bf 0}$$
\newpage

\begin{equation*}
    \Pi(x) = argmin_{w' = \Phi w} \|x - w'\|_{D}^{2} = argmin_{w} \|x - \Phi w\|_{D}^{2}
\end{equation*}
Therefore
\begin{equation*}
    -\Phi^{T}D(x - \Phi w^{\star})=0 
\end{equation*}
hence
\begin{equation*}
    \Pi(x) = \Phi(\Phi^{T}D\Phi)^{-1}\Phi^{T}Dx 
\end{equation*}
\begin{equation*}
    w^{t + 1} - w^{\star} = \gamma\left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP\Phi\left(w^{t} - w^{\star}\right).
\end{equation*}
We define $v^{t} = \Phi(w^{t} - w^{\star})$, then
\begin{equation*}
    v^{t + 1}= \gamma{\tilde A}v^{t} =  \gamma\Phi\left(\Phi^{T}D\Phi\right)^{-1}\Phi^{T}DP v^{t}.
\end{equation*}
Zico assumed the following
\begin{equation*}
    \|\Pi_{D}P\Phi w\|_{D} \leq \|\Phi w\|_{D},
\end{equation*}
which is equivalent to
\begin{equation*}
    \|\Phi(\Phi^{T}D\Phi)^{-1}\Phi^{T}DP\Phi w\|_{D} \leq \|\Phi w\|_{D},
\end{equation*}
so, in our terminology
\begin{equation*}
    \|{\tilde A}\Phi w\|_{D} \leq \|\Phi w\|_{D},
\end{equation*}
We have the following relation $\Phi A = {\tilde A}\Phi$. Moreover, ${\tilde A} = \Pi P$

\iffalse

, which is equivalent to $\Phi^{T}\Phi A = \Pi^{T}{\tilde A}\Phi$

Here, we will focus on the following class of algorithms:
\begin{equation} \label{Algo:Exact}
    w^{t + 1} \leftarrow \arg\min_{w} H_{t}(w),
\end{equation}
where (for the moment) we consider two options for the function $H$: 
\begin{itemize}
    \item[(i)] The vanilla TD class of algorithms $H_{t}(w) = h(w^{t} , w)$.
    \item[(ii)] The quadratic proximal TD class of algorithms $H_{t}(w) = h(w^{t} , w) + (1/2c_{t})\|w - w^{t}\|^{2}$, $c_{t} > 0$.
\end{itemize}
We begin with the proof of the exact approach, which is stated next.
\begin{theorem}[Contraction - Exact approach]
    Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by Algorithm \eqref{Algo:Exact}. Suppose that $w^{\star}$ is any point satisfying the condition $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$, then for any $t \in \mathbb{N}$, we have the following contraction property
    \begin{equation*}
        \|w^{t + 1} - w^{\star}\| \leq \eta\|w^{t} - w^{\star}\|,
    \end{equation*}
    where
    \begin{equation*}
        \eta = \begin{cases}
            L_{1}/\mu_2, & \text{case (i)}, \\
            (L_{1} + 1/c_{t})/\mu_{2}, & \text{case (ii)}.
        \end{cases}
    \end{equation*} 
\end{theorem}
\begin{proof}
From \eqref{Algo:Exact}, it immediately follows that $\nabla H_{t}(w^{t + 1}) = {\bf 0}$. Now, using the $\mu_{2}$-strong convexity of $w \rightarrow H_{t}(w)$, we get that
\begin{equation*}
    \mu_{2}\|w^{t + 1} - w^{\star}\|^{2} \leq \langle w^{\star} - w^{t + 1} , \nabla H_{t}(w^{\star}) - \nabla H_{t}(w^{t + 1}) \rangle = \langle w^{\star} - w^{t + 1} , \nabla H_{t}(w^{\star}) \rangle.
\end{equation*}
Now, since $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$, we obtain from the Cauchy-Schwartz inequality that
\begin{align*}
    \mu_{2}\|w^{t + 1} - w^{\star}\|^{2} & \leq \langle w^{\star} - w^{t + 1} , \nabla H_{t}(w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star}) \rangle \\
    & \leq \|w^{t + 1} - w^{\star}\| \cdot \|\nabla H_{t}(w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star})\|.
\end{align*}
Now, we split the proof to two cases. First, if $H_{t}(w) = h(w^{t} , w)$, we obtain that 
\begin{align*}
    \mu_{2}\|w^{t + 1} - w^{\star}\|^{2} & \leq \|w^{t + 1} - w^{\star}\| \cdot \|\nabla H_{t}(w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star})\| \\
    & \leq \|w^{t + 1} - w^{\star}\| \cdot \|\nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star})\| \\
    & \leq L_{1}\|w^{t + 1} - w^{\star}\| \cdot \|w^{t} - w^{\star}\|,    
\end{align*}
where the last inequality follows from the $L_{1}$-Lipschitz property of $\nabla_{2} h(\cdot,w^{\star})$. Second, if $H_{t}(w) = h(w^{t} , w) + (1/2c_{t})\|w - w^{t}\|^{2}$, we obtain from the triangle inequality that
\begin{align*}
    \|\nabla H_{t}(w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star})\| & = \|\nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star}) + (1/c_{t})(w^{\star} - w^{t})\| \\
    & \leq \|\nabla_{2} h(w^{t} , w^{\star}) - \nabla_{2} h(w^{\star} , w^{\star})\| + (1/c_{t})\|w^{t} - w{^\star}\| \\
    & \leq L_{1}\|w^{t} - w^{\star}\| + (1/c_{t})\|w^{t} - w{^\star}\| \\
    & = (L_{1} + 1/c_{t})\|w^{t} - w{^\star}\|,
\end{align*}
where the last inequality follows from the $L_{1}$-Lipschitz property of $\nabla_{2} h(\cdot,w^{\star})$.

Since this inequality holds true for any $t \in \mathbb{N}$, we see that if $w^{t} = w^{\star}$, then also $w^{t + 1} = w^{\ast}$. Thus, if $w^{T} = w^{\star}$ for some $T \in \mathbb{N}$, then $w^{t} = w^{\ast}$ for any $t \geq T$. On the other hand, if $w^{t} \neq w^{\ast}$ for all $t \in \mathbb{N}$, the desired result follows after dividing both sides by $\|w^{t + 1} - w^{\ast}\|$.
\end{proof}


Here, we will focus on the following class of algorithms:
\begin{equation} \label{Algo:Exact}
    w^{t + 1} \leftarrow \arg\min_{w} H_{t}(w),
\end{equation}
where (for the moment) we consider two options for the function $H$: 
\begin{itemize}
    \item[(i)] The vanilla TD class of algorithms $H_{t}(w) = h(w^{t} , w)$.
    \item[(ii)] The quadratic proximal TD class of algorithms $H_{t}(w) = h(w^{t} , w) + (1/2c_{t})\|w - w^{t}\|^{2}$, $c_{t} > 0$.
\end{itemize}
We begin with the proof of the exact approach, which is stated next.
\begin{theorem}[Contraction - Exact approach]
    Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by Algorithm \eqref{Algo:Exact}. Suppose that $w^{\star}$ is any point satisfying the condition $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$, then for any $t \in \mathbb{N}$, we have the following contraction property
    \begin{equation*}
        \|w^{t + 1} - w^{\star}\| \leq \eta\|w^{t} - w^{\star}\|,
    \end{equation*}
    where
    \begin{equation*}
        \eta = \begin{cases}
            L_{1}/\mu_2, & \text{case (i)}, \\
            (L_{1} + 1/c_{t})/\mu_{2}, & \text{case (ii)}.
        \end{cases}
    \end{equation*} 
\end{theorem}


In order to prove this result we will use the following basic result.
\begin{proposition} \label{P:Tech}
    Let $X, Y \in \mathbb{R}^{n \times n}$. If $\lambda_{min}(X) > \lambda_{max}(Y)$, then $X \succ Y$. Moreover, if $I \succ X$, then $\lambda_{max}(X) < 1$.
\end{proposition}
\begin{proof}
    From the basic definition of eigenvalue as an optimal solution for an optimization problem, we get the following
    \begin{align*}
        \lambda_{min}(X) > \lambda_{max}(Y) & \Leftrightarrow \min_{\|x\| = 1} x^{T}Xx > \max_{\|x\| = 1} x^{T}Yx \\
        & \Leftrightarrow \min_{\|x\| = 1} x^{T}Xx - \max_{\|x\| = 1} x^{T}Yx > 0 \\
        & \Leftrightarrow \min_{\|x\| = 1} x^{T}Xx + \min_{\|x\| = 1} - x^{T}Yx > 0 \\ 
        & \Rightarrow \min_{\|x\| = 1} x^{T}(X - Y)x > 0,        
    \end{align*}
    where the last inequality follows from the fact that $\min_{x} \{ f(x) + g(x) \} \geq \min_{x} f(x) + \min_{x} g(x)$. This proves the first desired result. 
    
    In order to prove the second item, we use the fact that $I - X \succ 0$, which means that all eigenvalues of $I - X$ are positive. Using again the definition of minimal eigenvalue we get that
    \begin{align*}
        0 < \lambda_{min}(I - X) = \min_{\|x\| = 1} x^{T}(I-X)x = \min_{\|x\| = 1} \{x^{T}Ix - x^{T}Xx\}= \min_{\|x\| = 1} \{1 - x^{T}Xx\} = 1 - \max_{\|x\| = 1} x^{T}Xx,        
    \end{align*}
    and thus $\lambda_{max}(X) < 1$ and the proof is completed.
\end{proof}
Now, we are ready to provide the following result.
\begin{corollary}
Let $\{ w^{t} \}_{t \in \mathbb{N}}$ be a sequence generated by TD and assume that $\gamma\|B\|_{2} < \lambda_{min}(C)$. Then, the sequence $\{ w^{t} \}_{t \in \mathbb{N}}$ converges to a solution $w^{\star}$ satisfying $\nabla_{2} h(w^{\star} , w^{\star}) = {\bf 0}$.
\end{corollary}
\begin{proof}
    From Proposition \ref{P:LinearTD} it is enough to show that in this case (recall that $\gamma \|B\|_{2} < \lambda_{min}(C)$), $\rho(A) < \gamma^{-1}$. For any matrix $X$ we have that $\rho(X) \leq \|X\|_{2}$, and therefore $\gamma\rho(B) \leq \gamma \|B\|_{2} < \lambda_{min}(C)$. From the definition of spectral radius it follows that $\gamma|\lambda_{i}(B)| < \lambda_{min}(C)$ for all $1 \leq i \leq n$. Using the fact that $\lambda_{max}(-X) = -\lambda_{min}(X)$, it means that $\gamma\lambda_{max}(\pm B) < \lambda_{min}(C)$. Using Proposition \ref{P:Tech}, it follows that $\gamma^{-1}I \succ \pm A$. Using again Proposition \ref{P:Tech}, it follows that $\lambda_{max}(A) < \gamma^{-1}$ and $-\lambda_{min}(A) = \lambda_{max}(-A) < \gamma^{-1}$. Therefore $\rho(A) < \gamma^{-1}$.
\end{proof}
We want to prove that $\lambda_{min}(A) > -\gamma^{-1}$. This is equivalent to proving that $\gamma^{-1} > -\lambda_{min}(A)$. Hence, we need to show that,
\begin{align*}
    \gamma^{-1} > -\lambda_{min}(A) & \Leftrightarrow \gamma^{-1} > -\min_{\|x\| = 1} x^{T}Ax \\
    & \Leftrightarrow \gamma^{-1} > \max_{\|x\| = 1} x^{T}(-A)x \\
    & \Leftrightarrow \gamma^{-1} > \lambda_{max}(-A)
\end{align*}

We actually want to prove that $L_{1} < \mu_{2}$ implies that $\gamma^{-1}I \succ \pm A$

\fi

==> tasks.tex <==
\section{Tasks}
\begin{itemize}
    \item {\bf Writing the proof for the non-prox setting}.
    \item {\bf Investigating the linear case with the squared loss as a special case of the theory}.
    \item Discussing the simple examples (2 examples from the book).  \\ http://www.incompleteideas.net/book/RLbook2020.pdf (section 11)
    \item what is known about convergence of TD? Kavosh: TD with linear function approximation and on-policy updates, we get convergence. Remove on-policy or lineraity and we will diverge.
    see this paper: 
    \href{https://www.mit.edu/~jnt/Papers/J063-97-bvr-td.pdf}{paper}
    \href{https://proceedings.neurips.cc/paper_files/paper/1996/file/e00406144c1e7e35240afed70f34166a-Paper.pdf}{paper}
    and this one \href{https://arxiv.org/abs/1904.10945}{paper}
    logistic Q learning \href{https://arxiv.org/pdf/2010.11151v1.pdf}{paper}
    \item what is different H?
    \item Check if the prox proof work with only convexity of $h$.
    \item Lihong suggests these papers:
    \href{http://www.machinelearning.org/archive/icml2008/papers/652.pdf}{melo}
    \href{https://www.jmlr.org/papers/volume9/munos08a/munos08a.pdf}{munos and csaba}
    \href{https://www.csd.uwo.ca/~dlizotte/publications/lizotte11convergent.pdf}{dan lizotte}
    \item {\bf Can we prove that strong convexity is must for convergence (in terms of contraction) of TD?}
    \item What is TD? Is it an algorithm? Is it a class of algorithms? RL people will think about it as the exact argmin of h? People will think about it as optimization algorithm?
\end{itemize}

